A Constructive Formalization of the Weak Perfect Graph Theorem

The Perfect Graph Theorems are important results in graph theory describing the relationship between clique number $\omega(G) $ and chromatic number $\chi(G) $ of a graph $G$. A graph $G$ is called \emph{perfect} if $\chi(H)=\omega(H)$ for every induced subgraph $H$ of $G$. The Strong Perfect Graph Theorem (SPGT) states that a graph is perfect if and only if it does not contain an odd hole (or an odd anti-hole) as its induced subgraph. The Weak Perfect Graph Theorem (WPGT) states that a graph is perfect if and only if its complement is perfect. In this paper, we present a formal framework for working with finite simple graphs. We model finite simple graphs in the Coq Proof Assistant by representing its vertices as a finite set over a countably infinite domain. We argue that this approach provides a formal framework in which it is convenient to work with different types of graph constructions (or expansions) involved in the proof of the Lov\'{a}sz Replication Lemma (LRL), which is also the key result used in the proof of Weak Perfect Graph Theorem. Finally, we use this setting to develop a constructive formalization of the Weak Perfect Graph Theorem.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

==> wpgt arxive/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> wpgt arxive/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

==> wpgt arxive/wpgtpic.tex <==

%%%%%% Triangle ABC
\newcommand{\UTriangle}
{
\path(0,0) coordinate (Origin);
\path (Origin)+ (0:0) coordinate(A) +(0: \d) coordinate(B) + (60: \d) coordinate(C);
\draw (A)--(B)--(C)--(A);
\node (a) at (A) [vertR] {};
\node (b) at (B) [vertB] {};
\node (c) at (C) [vertG] {};
}

%
%%%%%% Squares  ABCD
\newcommand{\USquare}
{
\path(2,0) coordinate (Origin);
\path(Origin) ++(0:0) coordinate(A) ++(0:\d) coordinate(B) ++ (90:\d) coordinate(C) ++ (180:\d) coordinate(D);
\draw (A)--(B)--(C)--(D)--(A);
\node (a) at (A)[vertR]{};
\node (b) at (B)[vertB]{};
\node (c) at (C)[vertR]{};
\node (d) at (D)[vertB]{};
}

%
%
%%%%%% Rectangles ABCD
\newcommand{\URectangle}
{
\path(0,0) coordinate (Origin);
\path(Origin) ++(0:0) coordinate(A) ++(0:\d+1) coordinate(B) ++ (90:\d) coordinate(C) ++ (180:\d+1) coordinate(D);
\draw (A)--(B)--(C)--(D)--(A);
\node (a) at (A)[vertR]{};
\node (b) at (B)[vertB]{};
\node (c) at (C)[vertR]{};
\node (d) at (D)[vertB]{};
}



%%%%%% Pentagon ABCDE
\newcommand{\UPentagon}
{
\path(0,0) coordinate (Origin);
\path (Origin) ++ (0:0) coordinate(Current);
\foreach \i in{0,1,2,...,4}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\draw (V0)--(V1)--(V2)--(V3)--(V4)--(V0);
\node (v0) at (V0) [vertR]{};
\node (v1) at (V1) [vertB]{};
\node (v2) at (V2) [vertR]{};
\node (v3) at (V3) [vertB]{};
\node (v4) at (V4) [vertG]{};
}

%%%%% Stars  ABCDE
\newcommand{\UStar}
{
\path(2,0) coordinate (Origin);
\path (Origin) ++ (0:0) coordinate(A) ++ (0:\d) coordinate(B) ++ (72:\d) coordinate(C) ++ (2*72:\d) coordinate(D) ++ (3*72:\d) coordinate(E);

\draw (A)--(C);
\draw (B)--(D);
\draw (C)--(E);
\draw (B)--(E);
\draw (A)--(D);
\node (a)[vertR] at (A){};
\node (b)[vertB] at (B){};
\node (c)[vertB] at (C){};
\node (d)[vertG] at (D){};
\node (e)[vertR] at (E){};
}

%%% Comp of House Graph
\newcommand{\UHouseComp}
{
\path(3,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}


% all the edges
\draw (V4)--(V1)--(V3)--(V5)--(V2);


\node (v1) at (V1) [vertB]{};
\node (v2) at (V2) [vertR]{};
\node (v3) at (V3) [vertR]{};
\node (v4) at (V4) [vertR]{};
\node (v5) at (V5) [vertB]{};
}


%%%%%%% Double Pentagon
\newcommand{\UDoublepentagon}
{
\path(5,0) coordinate (Origin);
\path (Origin) ++ (0:0) coordinate(Current);
\foreach \i in{0,1,2,...,4}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\draw (V0)--(V1)--(V2)--(V3)--(V4)--(V0);
\path(8,0)coordinate(Origin);
\path (Origin) ++ (0:0) coordinate(Current);
\foreach \i in{0,1,2,...,4}
{
\path (Current)++(0:0) coordinate(U\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\draw (U0)--(U1)--(U2)--(U3)--(U4)--(U0);
\draw (V2)--(U4)--(V3)--(U3)--(V2);
\node (v0) at (V0) [vertR]{};
\node (v1) at (V1) [vertB]{};
\node (v2) at (V2) [vertR]{};
\node (v3) at (V3) [vertB]{};
\node (v4) at (V4) [vertG]{};
\node (u0) at (U0) [vertC]{};
\node (u1) at (U1) [vertY]{};
\node (u2) at (U2) [vertC]{};
\node (u3) at (U3) [vertY]{};
\node (u4) at (U4) [vertBlack]{};
}


%%%%%%% Bipartite Graph

\newcommand{\UBipartitegraph}
{
\path(6,0)coordinate(Origin);
\def \dy  {\d/2}
\path(Origin) ++ (0,0) coordinate(l1) ++ (0,\dy) coordinate(l2) ++ (0,\dy) coordinate(l3) ++ (1,0) coordinate(r3) ++ (0,-\dy) coordinate(r2) ++ (0,-\dy) coordinate(r1);
\draw  (l1)--(r1);
\draw (l1)--(r2);
\draw (l2)--(r3);
\draw (l3)--(r2);

\node ()[vertR] at (l1){};
\node ()[vertR] at (l2){};
\node ()[vertR] at (l3){};

\node ()[vertB] at (r1){};
\node ()[vertB] at (r2){};
\node ()[vertB] at (r3){};
}



%%%%%% Line (M2)

\newcommand{\ULine}
{
\path (0,0) coordinate(Origin);
\path(Origin) +(0,0) coordinate(v1)+ (\d,0)coordinate(v2);
\draw(v1)--(v2);
\node ()[vertR] at(v1){};
\node ()[vertB] at(v2){};
}


%%%%%% Skewed Pentagon (M3)
\newcommand{\USkewedpentagon}
{
\path(0,0) coordinate(Origin);
\path(Origin) ++ (0:0) coordinate(A) ++ (0:\d) coordinate(B) ++ (1*72:\d) coordinate(C) ++ (2*72:\d) coordinate(D) ++ (3*72:\d) coordinate(E);
\draw (A)--(C)--(D)--(E)--(B)--(A);
\node() [vertR] at (A){};
\node() [vertG] at (B){};
\node() [vertB] at (C){};
\node() [vertR] at (D){};
\node() [vertB] at (E){};
}

%%%%%% Extended Pentagon
\newcommand{\UExtendedpentagon}
{
\path(0,0) coordinate (Origin);
\path (Origin) ++ (0:0) coordinate(Current);
\foreach \i in{0,1,2,...,4}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\path (V2) ++ (25:2*\d/3) coordinate (V5);
\draw (V0)--(V1)--(V2)--(V3)--(V4)--(V0);
\draw (V1)--(V5)--(V3);
\draw (V2)-- (V5);
\node (v0) at (V0) [vertR]{};
\node (v1) at (V1) [vertB]{};
\node (v2) at (V2) [vertR]{};
\node (v3) at (V3) [vertB]{};
\node (v4) at (V4) [vertG]{};
\node (v5) at (V5) [vertG]{};
}
%%%%%% graphs
\newcommand{\LGraph}
{ 
% Graph G 
\path(0,0) coordinate(Origin);
\path(Origin) ++ (0:0) coordinate(V2) ++ (5:0.7*\d) coordinate(V3) ++ (100:2*\d) coordinate(A) ++ (235:1.25*\d) coordinate(V1);
\draw (V2)--(A)--(V1);
\draw (V3)--(A);
\node (v2) at (V2) [vertBlack,label={below:{$v_{2}$}}]{};
\node (v3) at (V3) [vertBlack,label={below:{$v_{3}$}}]{};
\node (a) at (A) [vertBlack,label={above:{$a$}}]{};
\node (v1) at (V1) [vertBlack,label={below:{$v_{1}$}}]{};
\path (V2) ++ (280:1.5*\d) coordinate (G);
\node (g) at (G) []{$G$};

%% Graph G' by repeating vertex a to a'
\path(2.2*\d,0)coordinate(Origin);
\path(Origin) ++ (0:0) coordinate(V2) ++ (5:0.7*\d) coordinate(V3) ++ (100:2*\d) coordinate(A) ++ (235:1.25*\d) coordinate(V1);
\path (V3) ++ (75:1.1*\d) coordinate (A'); 
\draw (V2)--(A)--(V1);
\draw (V3)--(A);
\draw [thin,gray!40] (V2)--(A')--(V1);
\draw [thin,gray!40] (V3)--(A')--(A);
\node (v2) at (V2) [vertBlack,label={below:{$v_{2}$}}]{};
\node (v3) at (V3) [vertBlack,label={below:{$v_{3}$}}]{};
\node (a') at (A') [vertGB, label={right:{$a^{\prime}$}}]{};
\node (a) at (A) [vertBlack,label={above:{$a$}}]{};
\node (v1) at (V1) [vertBlack,label={below:{$v_{1}$}}]{};

\path (V2) ++ (280:1.5*\d) coordinate (G');
\node (g') at (G') []{$G'$};

%% Graph G'' by repeating vertex a' to a''
\path(5*\d,0)coordinate(Origin);
\path(Origin) ++ (0:0) coordinate(V2) ++ (5:0.7*\d) coordinate(V3) ++ (100:2*\d) coordinate(A) ++ (235:1.25*\d) coordinate(V1);
\path (V3) ++ (75:1.3*\d) coordinate (A'); 
\path (A') ++ (100:0.8*\d) coordinate (A'');
\draw (V2)--(A)--(V1);
\draw (V3)--(A);
\draw [thin,gray!40] (V2)--(A')--(V1);
\draw [thin,gray!40] (V3)--(A')--(A);

\draw [thin,gray!40] (V2)--(A'')--(V1);
\draw [thin,gray!40] (V3)--(A'')--(A);
\draw [thin,gray!40] (A'')--(A');

\node (v2) at (V2) [vertBlack,label={below:{$v_{2}$}}]{};
\node (v3) at (V3) [vertBlack,label={below:{$v_{3}$}}]{};
\node (a') at (A') [vertGB,label={right:{$a^{\prime}$}}]{};
\node (a'') at (A'') [vertGB, label={right:{$a^{\prime\prime}$}}]{};
\node (a) at (A) [vertBlack,label={above:{$a$}}]{};
\node (v1) at (V1) [vertBlack,label={below:{$v_{1}$}}]{};

\path (V2) ++ (280:1.5*\d) coordinate (G'');
\node (g'') at (G'') []{$G''$};
}


%%% Graph Expansion G and G'
\newcommand{\GenGExp}{
% %  Left polygon a - b - c - d
\path(0,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(D) ++ (0:1.5*\d) coordinate(C) ++ (90:\d) coordinate(B);
\path(origin) ++ (90:1.5*\d) coordinate(A);
\draw (D)--(C)--(B)--(A)--(D);
\node (d) at (D) [vertBlack,label={below left:{$d$}}]{};
\node (c) at (C) [vertBlack,label={below right:{$c$}}]{};
\node (b) at (B) [vertBlack,label={above right:{$b$}}]{};
\node (a) at (A) [vertBlack,label={above left:{$a$}}]{};

% label G at bottom
\path(origin) ++ (320:\d) coordinate(G);
\node (g) at (G) [label={below : {$G$}}]{};

%% the function g
\draw [->, thick] (4.2, 0.6*\d) to [out=170, in = 20] (2.8, 0.5*\d);
\node (fg) at (3.5, 0.6*\d) [label={above:{$g$}}]{};

%% Right extended polygon
\path(5,0) coordinate(origin);
\path(origin) ++ (0:0) coordinate(D) ++ (0:1.5*\d) coordinate(C) ++ (90:\d) coordinate(B);
\path(origin) ++ (90:1.5*\d) coordinate(A);
\path(A) ++ (30:0.25*\d) coordinate (A2);
\path(A) ++ (210:0.25*\d) coordinate (A1);
\path(D) ++ (270:0.2) coordinate (D1);
\path(C) ++ (0,0) coordinate (C1) ++ (0:0.5*\d) coordinate (C2) ++ (270:0.5*\d) coordinate (C3) ++ (180:0.5*\d) coordinate (C4);
\path(B) ++ (0:0) coordinate (B1) ++ (20:0.5*\d) coordinate (B2) ++ (140:0.5*\d) coordinate (B3);

%Edges between Va and Vb
\foreach \i in{1,2}
{
\foreach \j in {1,2,3}
{ \draw [gray!40](A\i)--(B\j); } 
}
%Edges between Vb and Vc
\foreach \i in{1,2,3}
{
\foreach \j in {1,2,3,4}
{ \draw [gray!40](B\i)--(C\j); } 
}
%Edges between Vc and Vd
\foreach \i in{1}
{
\foreach \j in {1,2,3,4}
{ \draw [gray!40](D\i)--(C\j); } 
}
%Edges between Vd and Va
\foreach \i in{1,2}
{
\foreach \j in {1}
{ \draw [gray!40](A\i)--(D\j); } 
}

\node (a1) at (A1) [vertBlack,label={above : {$V_{a}$}}]{};
\node (a2) at (A2) [vertBlack]{};
\node (b1) at (B1) [vertBlack]{};
\node (b2) at (B2) [vertBlack, label={above : {$V_{b}$}}]{};
\node (b3) at (B3) [vertBlack]{};
\node (c1) at (C1) [vertBlack]{};
\node (c2) at (C2) [vertBlack]{};
\node (c3) at (C3) [vertBlack, label={right : {$V_{c}$}}]{};
\node (c4) at (C4) [vertBlack]{};
\node (d1) at (D1) [vertBlack, label={below : {$V_{d}$}}]{};
\draw (A1)--(A2);
\draw (B1)--(B2)--(B3)--(B1);
\draw (C1)--(C2)--(C3)--(C4)--(C1)--(C3);
\draw (C2)--(C4);
% label G4 at bottom
\path(origin) ++ (320:\d) coordinate(G');
\node (g') at (G') [label={below : {$G'$}}]{};
}


%%% Vertices of a four sided polygon  a - b - c- d 
\newcommand{\LPolygonABCD}
{
\path(0,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(D) ++ (0:1.5*\d) coordinate(C) ++ (90:\d) coordinate(B);
\path(origin) ++ (90:1.5*\d) coordinate(A);
\draw (D)--(C)--(B)--(A)--(D);
\node (d) at (D) [vertBlack,label={below left:{$d$}}]{};
\node (c) at (C) [vertBlack,label={below right:{$c$}}]{};
\node (b) at (B) [vertBlack,label={above right:{$b$}}]{};
\node (a) at (A) [vertBlack,label={above left:{$a$}}]{};

% label G1 at bottom
\path(origin) ++ (320:\d) coordinate(G1);
\node (g1) at (G1) [label={below : {$G_{1}$}}]{};
}

%%%  Extended four-polygon Va-b-c-d
\newcommand{\LPolygonVaBCD}
{
\path (2.5,0) coordinate (Origin);
\path(Origin) ++ (0:0) coordinate(D) ++ (0:1.5*\d) coordinate(C) ++ (90:\d) coordinate(B);
\path(Origin) ++ (90:1.5*\d) coordinate(A);
\path(A) ++ (30:0.25*\d) coordinate (A2);
\path(A) ++ (210:0.25*\d) coordinate (A1);
%Edges between Vd and Va
\foreach \i in{1,2}
{
\draw [gray!40](A\i)--(D); 
}
% Edges between Va and b
\foreach \i in{1,2}
{
\draw [gray!40](A\i)--(B);  
}
\node (a1) at (A1) [vertBlack,label={above : {$V_{a}$}}]{};
\node (a2) at (A2) [vertBlack]{};
\node (b) at (B) [vertBlack, label={above : {$b$}}]{};
\node (c) at (C) [vertBlack, label={below : {$c$}}]{};
\node (d) at (D) [vertBlack, label={below : {$d$}}]{};
\draw (A1)--(A2);
\draw (D)--(C)--(B);
% label G2 at bottom
\path(Origin) ++ (320:\d) coordinate(G2);
\node (g2) at (G2) [label={below : {$G_{2}$}}]{};
}


%%% Extented four-polygon Va - Vb - c - d
\newcommand{\LPolygonVaVbCD}
{
\path(5,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(D) ++ (0:1.5*\d) coordinate(C) ++ (90:\d) coordinate(B);
\path(origin) ++ (90:1.5*\d) coordinate(A);
\path(A) ++ (30:0.25*\d) coordinate (A2);
\path(A) ++ (210:0.25*\d) coordinate (A1);
\path(B) ++ (0:0) coordinate (B1) ++ (20:0.5*\d) coordinate (B2) ++ (140:0.5*\d) coordinate (B3);
%Edges between Va and Vb
\foreach \i in{1,2}
{
\foreach \j in {1,2,3}
{ \draw [gray!40](A\i)--(B\j); } 
}
%Edges between Vb and c
\foreach \i in{1,2,3}
{
\draw [gray!40](B\i)--(C); 
}
%Edges between d and Va
\foreach \i in{1,2}
{
\draw [gray!40](A\i)--(D); 
}
\node (a1) at (A1) [vertBlack,label={above : {$V_{a}$}}]{};
\node (a2) at (A2) [vertBlack]{};
\node (b1) at (B1) [vertBlack]{};
\node (b2) at (B2) [vertBlack, label={above : {$V_{b}$}}]{};
\node (b3) at (B3) [vertBlack]{};
\node (c) at (C) [vertBlack, label={below : {$c$}}]{};
\node (d) at (D) [vertBlack, label={below : {$d$}}]{};
\draw (A1)--(A2);
\draw (B1)--(B2)--(B3)--(B1);
\draw (C)--(D);
% label G3 at bottom
\path(origin) ++ (320:\d) coordinate(G3);
\node (g3) at (G3) [label={below : {$G_{3}$}}]{};
}


%%% Extented four-polygon Va - Vb - Vc - Vd
\newcommand{\LExtendedpolygon}
{
\path(8,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(D) ++ (0:1.5*\d) coordinate(C) ++ (90:\d) coordinate(B);
\path(origin) ++ (90:1.5*\d) coordinate(A);
\path(A) ++ (30:0.25*\d) coordinate (A2);
\path(A) ++ (210:0.25*\d) coordinate (A1);
\path(D) ++ (270:0.2) coordinate (D1);
\path(C) ++ (0,0) coordinate (C1) ++ (0:0.5*\d) coordinate (C2) ++ (270:0.5*\d) coordinate (C3) ++ (180:0.5*\d) coordinate (C4);
\path(B) ++ (0:0) coordinate (B1) ++ (20:0.5*\d) coordinate (B2) ++ (140:0.5*\d) coordinate (B3);

%Edges between Va and Vb
\foreach \i in{1,2}
{
\foreach \j in {1,2,3}
{ \draw [gray!40](A\i)--(B\j); } 
}
%Edges between Vb and Vc
\foreach \i in{1,2,3}
{
\foreach \j in {1,2,3,4}
{ \draw [gray!40](B\i)--(C\j); } 
}
%Edges between Vc and Vd
\foreach \i in{1}
{
\foreach \j in {1,2,3,4}
{ \draw [gray!40](D\i)--(C\j); } 
}
%Edges between Vd and Va
\foreach \i in{1,2}
{
\foreach \j in {1}
{ \draw [gray!40](A\i)--(D\j); } 
}

\node (a1) at (A1) [vertBlack,label={above : {$V_{a}$}}]{};
\node (a2) at (A2) [vertBlack]{};
\node (b1) at (B1) [vertBlack]{};
\node (b2) at (B2) [vertBlack, label={above : {$V_{b}$}}]{};
\node (b3) at (B3) [vertBlack]{};
\node (c1) at (C1) [vertBlack]{};
\node (c2) at (C2) [vertBlack]{};
\node (c3) at (C3) [vertBlack, label={right : {$V_{c}$}}]{};
\node (c4) at (C4) [vertBlack]{};
\node (d1) at (D1) [vertBlack, label={below : {$V_{d}$}}]{};
\draw (A1)--(A2);
\draw (B1)--(B2)--(B3)--(B1);
\draw (C1)--(C2)--(C3)--(C4)--(C1)--(C3);
\draw (C2)--(C4);
% label G4 at bottom
\path(origin) ++ (320:\d) coordinate(G4);
\node (g4) at (G4) [label={below : {$G_{4}$}}]{};
}

%% Separating the overlaping sets in C
\newcommand{\GraphConstruct}
{
%% Overlaping stable sets
\path(2,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(B) ++ (90:2*\d) coordinate(A) ++ (90:0.8*\d) coordinate(Au);
\path(A) ++ (45: 0.8*\d) coordinate(Ar);
\path(A) ++ (135: 0.8*\d) coordinate(Al);
\path(B) ++ (45: 0.8*\d) coordinate(Br);
\path(B) ++ (135: 0.8*\d) coordinate(Bl);
% ellipse for Stable Sets
\path [fill= gray!10, rotate=135] (A) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (A) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=90] (A) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (B) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=135] (B) ellipse (25pt and 7pt);

\node (v1) at (Ar) [label={right :{$I_1$}}]{};
\node (v2) at (Au) [label={above :{$I_2$}}]{};
\node (v3) at (Al) [label={left :{$I_3$}}]{};
\node (v4) at (Br) [label={right:{$I_5$}}]{};
\node (v5) at (Bl) [label={left:{$I_4$}}]{};
\node (v6) at (B) [vertBlack,label={below:{$b$}}]{};
\node (v7) at (A) [vertBlack,label={below:{$a$}}]{};
% label C at bottom
\path(origin) ++ (270:0.7*\d) coordinate(C);
\node (c) at (C) [label={below : {$C$}}]{};

%% Separated stable sets
\path(6,0) coordinate (origin);
\path (origin) ++ (0:0) coordinate(Bl) ++ (0:1.5*\d) coordinate(Br)++(72:1.5*\d) coordinate(Ar);
\path (Ar) ++ (2*72:1.5*\d) coordinate(Au)++ (3*72:1.5*\d) coordinate(Al);

% ellipse for Stable Sets
\path [fill= gray!10, rotate=135] (Al) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (Ar) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=90] (Au) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (Bl) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=135] (Br) ellipse (25pt and 7pt);

\node (v1) at (Ar) [label={above right :{$I_{1}'$}}]{};
\node (v2) at (Au) [label={above left:{$I_{2}'$}}]{};
\node (v3) at (Al) [label={above left :{$I_{3}'$}}]{};
\node (v4) at (Br) [label={right:{$I_{4}'$}}]{};
\node (v5) at (Bl) [label={left:{$I_{5}'$}}]{};


\draw [gray!40](Al)--(Ar)--(Au)--(Al); 
\draw [gray!40](Bl)--(Br);

\node (v11) at (Ar) [vertBlack,label={below:{$(a,1)$}}]{};
\node (v22) at (Au) [vertBlack,label={right:{$(a,2)$}}]{};
\node (v33) at (Al) [vertBlack,label={below:{$(a,3)$}}]{};
\node (v44) at (Bl) [vertBlack,label={below:{$(b,5)$}}]{};
\node (v55) at (Br) [vertBlack,label={below:{$(b,4)$}}]{};
 
% label C' at bottom
\path(origin) ++ (320:\d) coordinate(C');
\node (c') at (C') [label={below : {$C'$}}]{};
}




%% Disjoint Stable Sets 
\newcommand{\LDisjStable}
{
\path(0,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(V1) ++ (0:1.5*\d) coordinate(V2) ++ (90:1.5*\d) coordinate(V3);
\path(origin) ++ (90:1.5*\d) coordinate(V4);
% ellipse for Stable Sets
\path [fill= gray!10, rotate=135] (V1) ellipse (23pt and 8pt);
\path [fill= gray!10, rotate=45] (V2) ellipse (23pt and 8pt);
\path [fill= gray!10, rotate=135] (V3) ellipse (23pt and 8pt);
\path [fill= gray!10, rotate=45] (V4) ellipse (23pt and 8pt);
%edges on clique
\foreach \i in {1,2,3,4}
{
\foreach \j in {1,2,3,4}
{ \draw [gray!40](V\i)--(V\j); } 
} 
\node (v1) at (V1) [vertBlack,label={below left:{$I_1$}}]{};
\node (v2) at (V2) [vertBlack,label={below right:{$I_2$}}]{};
\node (v3) at (V3) [vertBlack,label={above right:{$I_3$}}]{};
\node (v4) at (V4) [vertBlack,label={above left:{$I_4$}}]{};
% label G1 at bottom
\path(origin) ++ (320:\d) coordinate(G1);
\node (g1) at (G1) [label={below : {$G_{1}$}}]{};
}

%% Overlaping Stable Sets 
\newcommand{\LOverStable}
{
\path(4.5,0)coordinate(origin);
\path(origin) ++ (0:0) coordinate(B) ++ (90:2*\d) coordinate(A) ++ (90:0.8*\d) coordinate(Au);
\path(A) ++ (45: 0.8*\d) coordinate(Ar);
\path(A) ++ (135: 0.8*\d) coordinate(Al);
\path(B) ++ (45: 0.8*\d) coordinate(Br);
\path(B) ++ (135: 0.8*\d) coordinate(Bl);
% ellipse for Stable Sets
\path [fill= gray!10, rotate=135] (A) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (A) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=90] (A) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (B) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=135] (B) ellipse (25pt and 7pt);

\node (v1) at (Ar) [label={right :{$I_1$}}]{};
\node (v2) at (Au) [label={above :{$I_2$}}]{};
\node (v3) at (Al) [label={left :{$I_3$}}]{};
\node (v4) at (Br) [label={right:{$I_5$}}]{};
\node (v5) at (Bl) [label={left:{$I_4$}}]{};
\node (v6) at (B) [vertBlack,label={below:{$b$}}]{};
\node (v7) at (A) [vertBlack,label={below:{$a$}}]{};
% label G2 at bottom
\path(origin) ++ (270:0.7*\d) coordinate(G2);
\node (g2) at (G2) [label={below : {$G_{2}$}}]{};
}

%%% Seperated Stable Sets 
\newcommand{\LSepStable}
{
\path(8,0) coordinate (origin);
\path (origin) ++ (0:0) coordinate(Bl) ++ (0:1.5*\d) coordinate(Br)++(72:1.5*\d) coordinate(Ar);
\path (Ar) ++ (2*72:1.5*\d) coordinate(Au)++ (3*72:1.5*\d) coordinate(Al);

% ellipse for Stable Sets
\path [fill= gray!10, rotate=135] (Al) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (Ar) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=90] (Au) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=45] (Bl) ellipse (25pt and 7pt);
\path [fill= gray!10, rotate=135] (Br) ellipse (25pt and 7pt);

\node (v1) at (Ar) [label={above right :{$I_{1}'$}}]{};
\node (v2) at (Au) [label={above left:{$I_{2}'$}}]{};
\node (v3) at (Al) [label={above left :{$I_{3}'$}}]{};
\node (v4) at (Br) [label={right:{$I_{4}'$}}]{};
\node (v5) at (Bl) [label={left:{$I_{5}'$}}]{};


\draw [gray!40](Al)--(Ar)--(Au)--(Al); 
\draw [gray!40](Bl)--(Br);

\node (v11) at (Ar) [vertBlack,label={below:{$a_1$}}]{};
\node (v22) at (Au) [vertBlack,label={right:{$a_2$}}]{};
\node (v33) at (Al) [vertBlack,label={below:{$a_3$}}]{};
\node (v44) at (Bl) [vertBlack,label={below:{$b_1$}}]{};
\node (v55) at (Br) [vertBlack,label={below:{$b_2$}}]{};

 
% label G2' at bottom
\path(origin) ++ (320:\d) coordinate(G2);
\node (g2) at (G2) [label={below : {$G_{2}'$}}]{};
}


%%% Labelled Pentagon
\newcommand{\LPentagon}
{
\path(0,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\draw (V1)--(V2)--(V3)--(V4)--(V5)--(V1);
\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertR,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertB,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertG,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertR,label=below:{$v_{5}$}]{};
% label G1 at bottom
\path(Origin) ++ (300:\d) coordinate(G1);
\node (g1) at (G1) []{$G_{1}$};
}


%%% Labelled Pentagon with Cliques
\newcommand{\LPentagonWithIs}
{
\path(0,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}

\path (V1) ++ (72: 0.5*\d) coordinate (V12);
\path (V4) ++ (4*72: 0.5*\d) coordinate (V45);
% ellipse for cliques
\path [fill= gray!10, rotate=72] (V12) ellipse (23pt and 7pt);
\path [fill= gray!10, rotate=108] (V45) ellipse (23pt and 7pt);
\path [fill= gray!10, rotate=0] (V3) ellipse (17pt and 7pt);
\node (v12) at (V12) [label=right:{$I_{1}$}]{};
\node (v45) at (V45) [label=left:{$I_{3}$}]{};
\node (v3n) at (V3) [label=right:{$I_{2}$}]{};

% all the edges
\draw (V1)--(V2)--(V3)--(V4)--(V5)--(V1);


\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertR,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertB,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertG,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertR,label=below:{$v_{5}$}]{};
% label G1 at bottom
\path(Origin) ++ (300:\d) coordinate(G1);
\node (g1) at (G1) []{$G$};
}

%%%%% Labeled Star with Stable sets 
\newcommand{\LStarWithIs}
{
%identifying coordinates for vertices
\path(4,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}

\path (V1) ++ (72: 0.5*\d) coordinate (V12);
\path (V4) ++ (4*72: 0.5*\d) coordinate (V45);
% puting ellipse and label for stable sets
\path [fill= gray!10, rotate=72] (V12) ellipse (23pt and 7pt);
\path [fill= gray!10, rotate=108] (V45) ellipse (23pt and 7pt);
\path [fill= gray!10, rotate=0] (V3) ellipse (17pt and 7pt);
\node (v12) at (V12) [label=right:{$I_{1}$}]{};
\node (v45) at (V45) [label=left:{$I_{3}$}]{};
\node (v3n) at (V3) [label=right:{$I_{2}$}]{};

% all the edges
\draw (V1)--(V3)--(V5)--(V2)--(V4)--(V1);

%labels and colours on vertices
\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertB,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertG,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertR,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertR,label=below:{$v_{5}$}]{};
% label G2 at bottom
\path(Origin) ++ (300:\d) coordinate(G2);
\node (g2) at (G2) []{$G'$};

}

%%% Labelled House Graph
\newcommand{\LHouse}
{
\path(0,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}


% all the edges
\draw (V1)--(V2)--(V3)--(V4)--(V5)--(V1);
\draw (V2)--(V4);


\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertR,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertB,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertG,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertR,label=below:{$v_{5}$}]{};
% label G1 at bottom
\path(Origin) ++ (300:\d) coordinate(G1);
\node (g1) at (G1) []{$G$};
}

%%% Labelled Comp of House Graph
\newcommand{\LHouseComp}
{
\path(4,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}


% all the edges
\draw (V4)--(V1)--(V3)--(V5)--(V2);


\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertR,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertR,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertR,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertB,label=below:{$v_{5}$}]{};
% label G1 at bottom
\path(Origin) ++ (300:\d) coordinate(G1);
\node (g1) at (G1) []{$G'$};
}



%%% Labelled pentagon obtained by repeating vertex v4
\newcommand{\LExtendedpentagon}
{
\path(3,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\path(V4) ++ (340:0.3*\d) coordinate(V4');
\draw (V1)--(V2)--(V3)--(V4)--(V5)--(V1);
\draw (V3)--(V4')--(V5);
\draw (V4)--(V4');
\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertG,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertR,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertB,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertR,label=below:{$v_{5}$}]{};
\node (v4') at (V4') [vertG,label=right:{$v_{4}^{\prime}$}]{};
% label G2 at bottom
\path(Origin) ++ (300:\d) coordinate(G2);
\node (g2) at (G2) []{$G_{2}$};
}
%
%
%%% Labelled pentagon obtained by repeating vertex v4 and v2

\newcommand{\LDextendedpentagon}
{
\path(6,0) coordinate (Origin);
\path (Origin) ++ (0:\d) coordinate(Current);
\foreach \i in{1,2,...,5}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\path(V4) ++ (340:0.3*\d) coordinate(V4');
\path(V2) ++ (200:0.3*\d) coordinate(V2');
\draw (V1)--(V2)--(V3)--(V4)--(V5)--(V1);
\draw (V3)--(V4')--(V5);
\draw (V4)--(V4');
\draw (V3)--(V2')--(V1);
\draw (V2)--(V2');
\node (v1) at (V1) [vertB,label=below:{$v_{1}$}]{};
\node (v2) at (V2) [vertG,label=right:{$v_{2}$}]{};
\node (v3) at (V3) [vertR,label=above:{$v_{3}$}]{};
\node (v4) at (V4) [vertB,label=left:{$v_{4}$}]{};
\node (v5) at (V5) [vertR,label=below
:{$v_{5}$}]{};
\node (v4') at (V4') [vertG,label=right:{$\scriptstyle{v_{4}^{\prime}}$}]{};
\node (v2') at (V2') [vertC,label=left:{$\scriptstyle{v_{2}^{\prime}}$}]{};

% label G3 at bottom
\path(Origin) ++ (300:\d) coordinate(G3);
\node (g3) at (G3) []{$G_{3}$};
}

%%% pentagon and square joined
\newcommand{\Pentagonsquare}
{
\path(3,0) coordinate (Origin);
\path (Origin) ++ (0:0) coordinate(Current);
\foreach \i in{0,1,2,...,4}
{
\path (Current)++(0:0) coordinate(V\i);
\path (Current)++(\i*72: \d) coordinate(Current);
}
\draw (V0)--(V1)--(V2)--(V3)--(V4)--(V0);
\node (v0) at (V0) [vertR]{};
\node (v1) at (V1) [vertB]{};
\node (v2) at (V2) [vertR]{};
\node (v3) at (V3) [vertB]{};
\node (v4) at (V4) [vertG]{};
\path(5,0.3) coordinate (Origin);
\path(Origin) ++(0:0) coordinate(A) ++(0:\d) coordinate(B) ++ (90:\d) coordinate(C) ++ (180:\d) coordinate(D);
\draw (A)--(B)--(C)--(A)--(D)--(B);
\draw(C)--(D);
\draw(V2)--(D);
\node (a) at (A)[vertG,scale=1]{};
\node (b) at (B)[vertR,scale=1]{};
\node (c) at (C)[vertB,scale=1]{};
\node (d) at (D)[vertC,scale=1]{};
}





